Dimension-independent rates for structured neural density estimation

We show that deep neural networks achieve dimension-independent rates of convergence for learning structured densities such as those arising in image, audio, video, and text applications. More precisely, we demonstrate that neural networks with a simple $L^2$-minimizing loss achieve a rate of $n^{-1/(4+r)}$ in nonparametric density estimation when the underlying density is Markov to a graph whose maximum clique size is at most $r$, and we provide evidence that in the aforementioned applications, this size is typically constant, i.e., $r=O(1)$. We then establish that the optimal rate in $L^1$ is $n^{-1/(2+r)}$ which, compared to the standard nonparametric rate of $n^{-1/(2+d)}$, reveals that the effective dimension of such problems is the size of the largest clique in the Markov random field. These rates are independent of the data's ambient dimension, making them applicable to realistic models of image, sound, video, and text data. Our results provide a novel justification for deep learning's ability to circumvent the curse of dimensionality, demonstrating dimension-independent convergence rates in these contexts.

==> simple-graph-examples.tex <==
\begin{wrapfigure}{R}{0.4\textwidth}
    \centering
    \begin{tikzpicture}[scale=0.5]
    % Draw the nodes
    \node (n1) at (0,1) [circle, draw] {};
    \node (n2) at (1,1) [circle, draw] {};
    \node (n3) at (2,1) [circle, draw] {};
    \node (n4) at (3,1) [circle, draw] {};

    % Draw the edges
    \draw (n1) -- (n2);
    \draw (n2) -- (n3);
    \draw (n3) -- (n4);

    % Label the nodes
    % \node at (n1) [below] {1};
    % \node at (n2) [below] {2};
    % \node at (n3) [below] {3};
    % \node at (n4) [below] {4};

    % Add the path label
    % \node at (1.5, -1) {path / $r=\log d$ / $n \gtrsim (1/\epsilon)^{\log d}$};
    \node at (1.5, -1)[align=center] {{\bf Path} ($L_4$)};
\end{tikzpicture}~
\begin{tikzpicture}[scale=0.5]
    % Draw the nodes
    \node (n1) at (0,0) [circle, draw] {};
    \node (n2) at (1,0) [circle, draw] {};
    \node (n3) at (2,0) [circle, draw] {};
    \node (n4) at (0,1) [circle, draw] {};
    \node (n5) at (1,1) [circle, draw] {};
    \node (n6) at (2,1) [circle, draw] {};
    \node (n7) at (0,2) [circle, draw] {};
    \node (n8) at (1,2) [circle, draw] {};
    \node (n9) at (2,2) [circle, draw] {};

    % Draw the edges
    \draw (n1) -- (n2);
    \draw (n2) -- (n3);
    \draw (n4) -- (n5);
    \draw (n5) -- (n6);
    \draw (n7) -- (n8);
    \draw (n8) -- (n9);
    \draw (n1) -- (n4);
    \draw (n4) -- (n7);
    \draw (n2) -- (n5);
    \draw (n5) -- (n8);
    \draw (n3) -- (n6);
    \draw (n6) -- (n9);

    % Add the grid label
    % \node at (1, -1) {grid / $r=\sqrt{d}$ / $n \gtrsim (1/\epsilon)^{\sqrt{d}}$};
    \node at (1, -1)[align=center] {{\bf Grid} ($L_{3\times 3}$)};
\end{tikzpicture}
\begin{tikzpicture}[scale=0.5]
    \node (n1) at (0,0) [circle, draw] {};
    \node (n2) at (1,0) [circle, draw] {};
    \node (n3) at (2,0) [circle, draw] {};
    \node (n4) at (0,1) [circle, draw] {};
    \node (n5) at (1,1) [circle, draw] {};
    \node (n6) at (2,1) [circle, draw] {};
    \node (n7) at (0,2) [circle, draw] {};
    \node (n8) at (1,2) [circle, draw] {};
    \node (n9) at (2,2) [circle, draw] {};
    % Draw the edges
    \draw (n1) -- (n2) -- (n3) -- (n6) -- (n9) -- (n8) -- (n7) -- (n4) -- (n1);
    \draw (n4) -- (n5) -- (n6);
    \draw (n2) -- (n5) -- (n8);
    % Draw the diagonal edges
    \draw (n1) -- (n5) -- (n9);
    \draw (n3) -- (n5) -- (n7);
    \draw (n2) -- (n4);
    \draw (n2) -- (n6);
    \draw (n4) -- (n8);
    \draw (n6) -- (n8);
    % Add the grid label
    \node at (1, -1)[align=center] {{\bf Grid with Diagonals} ($L_{3\times 3}^+$)};
\end{tikzpicture}
\caption{\emph{Highly simplified} examples of common MRF graphs. Paths correspond to sequential data and grids to spatial.}
\label{fig:simple-graph-examples}
\end{wrapfigure}
